Unsupervised Polychromatic Neural Representation for CT Metal Artifact Reduction

Emerging neural reconstruction techniques based on tomography (e.g., NeRF, NeAT, and NeRP) have started showing unique capabilities in medical imaging. In this work, we present a novel Polychromatic neural representation (Polyner) to tackle the challenging problem of CT imaging when metallic implants exist within the human body. CT metal artifacts arise from the drastic variation of metal's attenuation coefficients at various energy levels of the X-ray spectrum, leading to a nonlinear metal effect in CT measurements. Recovering CT images from metal-affected measurements hence poses a complicated nonlinear inverse problem where empirical models adopted in previous metal artifact reduction (MAR) approaches lead to signal loss and strongly aliased reconstructions. Polyner instead models the MAR problem from a nonlinear inverse problem perspective. Specifically, we first derive a polychromatic forward model to accurately simulate the nonlinear CT acquisition process. Then, we incorporate our forward model into the implicit neural representation to accomplish reconstruction. Lastly, we adopt a regularizer to preserve the physical properties of the CT images across different energy levels while effectively constraining the solution space. Our Polyner is an unsupervised method and does not require any external training data. Experimenting with multiple datasets shows that our Polyner achieves comparable or better performance than supervised methods on in-domain datasets while demonstrating significant performance improvements on out-of-domain datasets. To the best of our knowledge, our Polyner is the first unsupervised MAR method that outperforms its supervised counterparts. The code for this work is available at: https://github.com/iwuqing/Polyner.

==> table/table_loss_eas.tex <==
\begin{table}
\centering
\caption{Quantitative results of the proposed PolyNeRF model over the loss $\mathcal{L}_\text{EAS}$ on the DeepLesion \cite{deeplesion} dataset.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lc} 
\toprule
Hyper-Parameter & PSNR \\ \midrule
$\lambda = 0$ & 22.71$\pm$4.97\\
$\lambda = 0.1$ & 33.75$\pm$2.30\\
$\lambda = 0.2$ & \textbf{36.87$\pm$1.56}\\
$\lambda = 0.3$ & 36.83$\pm$1.52\\
$\lambda = 0.4$ & 36.39$\pm$1.79\\
\bottomrule
\end{tabular}}
\end{table}


==> table/table_real.tex <==
\begin{table}
\centering
\caption{Quantitative results of the compared methods on our collected walnut sample. The best and second performances are respectively highlighted in \textbf{bold} and \underline{underline}.}
\label{table_real}
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{0.25cm}{
\begin{tabular}{ccccccc} 
\toprule
 & FBP \cite{fbp} & LI \cite{kalender1987li} & ACDNet \cite{wang2022acdnet} & DIDCNet \cite{wang2021dicdnet} & Score-MAR \cite{song2022solving} & Polyner (Ours) \\ \midrule
PSNR & 20.66 & \underline{21.94} & 21.53 & 21.61 & 10.36 & \textbf{22.00} \\
SSIM & 0.3623  & \underline{0.4853} & 0.3592 & 0.3562 & 0.2745 & \textbf{0.5484} \\ 
\bottomrule
\end{tabular}}}
\end{table}

% \begin{table}
% \centering
% \caption{Quantitative results of the compared methods on our collected walnut sample. The best and second performances are respectively highlighted in \textbf{bold} and \underline{underline}.}
% \label{table_real}
% \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccccc} 
% \toprule
%  & FBP \cite{fbp} & LI \cite{kalender1987li} & ACDNet \cite{wang2022acdnet} & DIDCNet \cite{wang2021dicdnet} & Score SDE \cite{song2022solving} & Polyner (Ours) \\ \midrule
% PSNR & 20.70 & \underline{21.96} & 21.55 & 21.61 && \textbf{22.02} \\
% SSIM & 0.3637  & \underline{0.4854} & 0.3605 & 0.3570 && \textbf{0.5497} \\ 
% \bottomrule
% \end{tabular}}
% \end{table}
